RoadTrack: Realtime Tracking of Road Agents in Dense and Heterogeneous Environments

We present a realtime tracking algorithm, RoadTrack, to track heterogeneous road-agents in dense traffic videos. Our approach is designed for traffic scenarios that consist of different road-agents such as pedestrians, two-wheelers, cars, buses, etc. sharing the road. We use the tracking-by-detection approach where we track a road-agent by matching the appearance or bounding box region in the current frame with the predicted bounding box region propagated from the previous frame. RoadTrack uses a novel motion model called the Simultaneous Collision Avoidance and Interaction (SimCAI) model to predict the motion of road-agents by modeling collision avoidance and interactions between the road-agents for the next frame. We demonstrate the advantage of RoadTrack on a dataset of dense traffic videos and observe an accuracy of 75.8% on this dataset, outperforming prior state-of-the-art tracking algorithms by at least 5.2%. RoadTrack operates in realtime at approximately 30 fps and is at least 4 times faster than prior tracking algorithms on standard tracking datasets.

==> append.tex <==
\clearpage
\section*{Appendix: Reduced Probability of Track Loss with Background Subtracted Object Representation}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% \newtheorem{prop}{Proposition}
% \newtheorem{thm}{Theorem}
% \newtheorem{lemma}{Lemma}
% \crefname{lemma}{Lemma}{Lemmas}
% \newcommand{\xpi}[1]{#1_{p_i}}
% \newcommand{\xhj}[1]{#1_{h_j}}
% \newcommand{\msk}{f^M_{h_j}}
% \newcommand{\fst}{f^F_{h_j}}
% \newcommand{\ft}{f^T_{\p}}
% \newcommand{\p}{p_i}
% \newcommand{\h}{h_j}
% \newcommand{\ith}{i^{\textrm{th}}}
% \newcommand{\jth}{j^{\textrm{th}}}
% \newcommand{\tim}[1]{\textrm{#1}}
% \newcommand{\mc}[1]{\mathcal{#1}}
% \newcommand{\bb}[1]{\mathbb{#1}}
% \newcommand{\utt}[1]{\textcolor{red}{#1}}

% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% % \begin{document}

% \maketitle

\noindent In this report, we consider Mask R-CNN for road-agent detection, which outputs bounding boxes and their corresponding masks. We define $\mc{T}_{t} =\{\Psi_{1:t}\}$ to be the set of positively identified states for agent $\p$ until time $t$. We denote the time since the last update to a track ID as $\mu$. We denote the ID of $\p$ as $\alpha$ and we represent the correct assignment of an ID to $\p$ as $\Gamma(\alpha)$. The threshold for the Cosine metric is $\lambda \underset{\tim{i.i.d.}}{\sim} \bb{U}[0,1]$. The threshold for the track age, \textit{i.e.}, the number of frames before which track is destroyed, is $\xi$. We denote the probability of an event that uses Mask R-CNN as the primary object detection algorithm with $\bb{P}^M(\cdot)$ and the probability of an event that uses a standard Faster R-CNN as the primary object detection algorithm (\textit{i.e.}, outputs bounding boxes without background subtraction) with $\bb{P}^F(\cdot)$. Finally, $\mc{T}_{t} \gets \{\phi\}$ represents the loss of $\mc{T}_{t}$ by occlusion.



% Based on Lemma~\ref{lemma1}, we finally prove the following proposition.
\begin{thm}
With probability $1-\frac{B}{A}$, binary tensors extracted from the background subtracted (BGS) representations decrease the number of road agent tracks lost, thereby reducing the number of false negatives, in comparison to regular bounding boxes.
\label{thm}
\end{thm}
% \vspace{-10pt}
\begin{proof} We use the mask from Mask-RCNN and bounding box pair to generate a BGS representation. The correct assignment of an ID depends on successful feature matching between the predicted measurement feature and the optimal detection feature. In other words, 

\begin{equation}
\mathnormal{l}(\xpi{f},f_{h^{*}_j})>\lambda \Leftrightarrow (\alpha = \phi)
\label{eqn:assign}
\end{equation} 

\noindent Using Proposition~\ref{lemma} and the fact that $\lambda \underset{i.i.d.}{\sim} \bb{U}[0,1]$, 
\[\bb{P}(\mathnormal{l}(\xpi{f} , f^M_{h^{*}_{j,\p}} ) > \lambda) < \bb{P}(\mathnormal{l}(\xpi{f} ,f^F_{h^{*}_{j,\p}} ) > \lambda)\] 
\noindent Using Eq. 1, it directly follows that,
\begin{equation}
    \bb{P}^M(\alpha = \phi) < \bb{P}^F(\alpha = \phi)
    \label{alpha}
\end{equation}

\noindent In our approach, we set \[(\mu>\xi) \land  (\alpha = \phi) \Leftrightarrow \mc{T}_{t} \gets \{\phi\}\]
Using Eq.~2, it follows that,
\begin{equation}
\bb{P}^M(\mc{T}_{t} \gets \{\phi\}) < \bb{P}^F(\mc{T}_{t} \gets \{\phi\})
\label{prob}
\end{equation}
We define the total number of false negatives (FN) as 
\begin{equation}
    FN = \sum_{t=1}^T \sum_{p_g \in \mc{G}} \delta_{\mc{T}_{t}}
    \label{fn}
\end{equation}
where $p_g \in \mc{G}$ denotes a ground truth pedestrian in the set of all ground truth pedestrians at current time $t$ and $\delta_z = 1$ for $z=0$ and $0$ elsewhere. This is a variation of the Kronecker delta function.
Using Eq.~3 and Eq.~4, we can say that fewer lost tracks ($\mc{T}_{t} \gets \{\phi\}$) indicate a smaller number of false negatives. 
% \hfill $\blacksquare$

% Finally, by using Lemma \ref{lemma1} with the association formulation Eq.~\ref{optim} described in the next subsection, it is easy to see that $\bb{P}^M(\Gamma(\alpha))>\bb{P}^F(\Gamma(\alpha))$, 

% which completes the proof.
\end{proof}

\noindent The upper bound, $\bb{P}^F(\mc{T}_{t})$, in Eq.~3 depends on the amount of padding done to $\xpi{f}$ and $\xhj{f}$. A general observed trend is that a higher amount of padding results in a larger upper bound in Eq.~3.



% We now state and prove the following lemma.
\begin{prop}
For every pair of binary tensors $(\msk, \fst)$ generated from a BGS-Representation and a bounding box respectively, if $\lVert\msk\lVert_0 > \lVert\fst\rVert_0$, then $\mathnormal{l}(\xpi{f},\msk) < \mathnormal{l}(\xhj{f},\fst) $ with probability $1 - \frac{c_1}{c_2}$, where $A$ and $B$ are positive integers and $c_1 > c_2$.
\label{lemma}
\end{prop}
% \vspace{-5pt}
\begin{proof}
Using the definition of the Cosine metric, the lemma reduces to proving the following,

\begin{equation}
\xpi{f}^T(\msk - \fst) > 0
\label{diseq1}
\end{equation}

\noindent We pad both $\msk$ and $\fst$ such that $\lVert\msk\rVert_0 > ||\fst||_0$.\\

\noindent We reduce $\ft$, $\msk$, and $\fst$ to binary vectors, \textit{i.e.}, vectors composed of $0$s and $1$s. Let $\Delta f = \msk - \fst$. We denote the number of $1$s and $-1$s in $\Delta f$ as $c_1$ and $c_2$, respectively. Now, let $x$ and $y$ denote the $L_0$ norm of $\msk$ and $\fst$, respectively. From our padding procedure, we have $x>y$. Then, if $x=c_1$, and $y=c_2$, we trivially have $A>B$. But if $y>c_2$, then $c_1= x-(y-c_2) \implies c_1 - c_2 = x - y$. From $x>y$, it again follows that $c_1>c_2$. Thus, $x>y \implies c_1>c_2$.\\

\noindent Next, we define a $(1,1)$ coordinate in an ordered pair of vectors as the coordinate where both vectors contain $1$s. Similarly, a $(1,-1)$ coordinate in an ordered pair of vectors is the coordinate where the first vector contains $1$ and the second vector contains $-1$. Then, let $p_a$ and $p_b$ respectively denote the number of $(1,1)$ coordinates and $(1,-1)$ coordinates in the pair $(\ft,\Delta f)$. By definition, we have $0<p_a<c_1$ and $0<p_b<c_2$. Thus, if we assume $p_a$ and $p_b$ to be uniformly distributed, it directly follows that $\bb{P}(p_a>p_b) = 1-\frac{c_2}{c_1}$. 
% \hfill $\blacksquare$


\end{proof}


% \end{document}


 

==> comp_datasets.tex <==
% \begin{table*}[t]
%   \centering
% %   \scalebox{0.7}{
%   \begin{tabular}{|c|c|p{.3cm}|p{0.35cm}|c|p{0.3cm}|c|p{0.45cm}|c|c|}
%   \hline
%     Dataset (\# classes) & Person &Car & Bike & Scooter & Bus & Truck & Cycle & Rickshaw &Animal\\
%     \hline
%     KITTI(3) &9.5 &2 &0 &0 &0 &0 &0 &1.5 &0\\
%     MOT (3) &13 &3 &0 &0 &0.5 &0 &0 &0  &0\\
%     PETS09 (2) &13 &0 &0 &0 &0 &0.5 &0 &0 &0\\
%     \hline
%     \textbf{Our Dataset (8)} &\textbf{28.5} &\textbf{37} &\textbf{22} &\textbf{8} &\textbf{2} &\textbf{0.5} &\textbf{1.5} &\textbf{14.5} &\textbf{1}\\
%     \hline
%   \end{tabular}
% %   }
%   \caption{We pick the top two sequences of various traffic datasets and compare heterogeneity with ours (TRAF11 and TRAF12). We observe a high variety of traffic agents.}
% \vspace{-20pt}
%   \label{table2}
% \end{table*}

\begin{table*}
    \centering
    \scalebox{0.9}{
  \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
    \multirow{2}{*}{Dataset} & \# Frames & \multicolumn{9}{c|}{Agents} & Visibility & Density & \#Diff \\
    \cline{3-11}
    & $(\times 10^3)$ & Ped & Bicycle & Car & Bike & Scooter & Bus & Truck & Rick & Total & (Km) & $(\times 10^{3})$ & Agents \\
    \hline
    KITTI-16$^*$ & 8.4 & 9.5 & 0.2 & 1.8 & 0 & 0 & 0.1 & 0.1 & 0 & 11.7 & 0.200 & 0.06 & 3\\
    \hline
    PETS09$^*$ & 0.8 & 13 & 0 & 0 & 0 & 0 & 0.5 & 0 & 0 & 13.5 & 0.150 & 0.09 & 2\\
    \hline
    NGSIM & 10.2 & 0 & 0 & 981.4 & 3.9 & 0 & 0 & 28.2 & 0 & 1013.5 & 0.548 & 1.85 & 3\\
    \hline
    Beijing$^*$ & 93 & 1.6 & 1.9 & \multicolumn{6}{c|}{12.9} & 16.4 & 0.005 & 3.28 & 3\\
    \hline
    \textbf{TRAF$^*$} & 12.4 & 4.9 & 1.5  &3.6 & 1.43 & 5 & 0.15 & 0.2 & 3.1 & 19.88 & 0.005 & 3.97 & 8 \\
    \hline
  \end{tabular}
  }
    \caption{Comparison of our new TRAF dataset with various traffic datasets in terms of heterogeneity and density of traffic agents. Heterogeneity is described in terms of the number of different agents that appear in the overall dataset. Density is the total number of traffic agents per Km in the dataset. The value for each agent type under ``Agents'' corresponds to the average number of instances of that agent per frame of the dataset. It is computed by taking all the instances of that agent and dividing by the total number of frames. Visibility is a ballpark estimate of the length of road in meters that is visible from the camera. NGSIM data were collected using tower-mounted cameras (bird's eye view), whereas both Beijing and TRAF data presented here were collected with car-mounted cameras (frontal view). For datasets marked with $^*$, the values in their corresponding rows are computed using only a representative subset of those datasets and are an approximation of the true values for the entire dataset.}
    \label{dataset}
\end{table*}


==> feature_extraction.tex <==
% \subsection{Feature Extraction Using Segmented Representations}
\label{sec4B}
% We extract simple, yet powerful, tensors, called ??, from segmented shapes, that are obtained from Mask R-CNN, using a convolutional neural network. The architectural and training details of this network are described in \cite{deepsort}. 
% % Deep TA-Features are grid-like maps that are stacked in a pyramid-shaped structure. Each layer of this pyramid encodes a visual aspect (for example, facial features or vehicle parts) of a traffic agent.
% We present a formulation in which ??? features significantly improve the performance of our algorithm by reducing false negatives, (ground truth agents that are not tracked). These often arise in dense scenarios due to increased instances of collisions and interactions. 

% \subsection{Analysis}
% \label{sec4B}
% We present a formulation in which binary tensors significantly improve the performance of our algorithm by reducing false negatives, (ground truth agents that are not tracked). These often arise in dense scenarios due to increased instances of collisions and interactions. 

% We define $\mc{T}_{t} =\{\Psi_{1:t}$ to be the set of positively identified states for $\p$ until time $t$. We denote the time since the last update to a track ID as $\mu$. We denote the ID of $\p$ as $\alpha$ and we represent the correct assignment of an ID to $\p$ as $\Gamma(\alpha)$. The threshold for the cosine distance is $\lambda \underset{\tim{i.i.d.}}{\sim} \bb{U}[0,1]$. The threshold for the track age, that is, the threshold for number of frames before which track is destroyed, is $\xi$. We denote the probability of an event (or process) that uses Mask R-CNN as the object detection algorithm with $\bb{P}^M(\cdot)$ and the probability of an event (or process) that uses Faster R-CNN as the main object detection algorithm with $\bb{P}^F(\cdot)$. $\bb{P}$ without a superscript denotes general probability. Finally, $\mc{T}_{t} \gets \{\phi\}$ represents the loss of $\mc{T}_{t}$ by occlusion.


% \begin{lemma}
% For every pair of binary tensors, $(\msk, \fst)$ generated from a BS-representation and a bounding box respectively, if $||\msk||_0 > ||\fst||_0$, then $\mathnormal{d}(\xpi{f},\msk) < \mathnormal{d}(\xhj{f},\fst) $ with probability $1 - B/A$.
% \label{lemma1}
% \end{lemma}
% \vspace{-5pt}
% \begin{proof}

% Using the definition of the cosine distance, we can reduce our problem to proving the following,

% \begin{equation}
% \xpi{f}^T(\msk - \fst) > 0
% \label{diseq1}
% \end{equation}

% \noindent We pad both $\msk$ and $\fst$ such that $||\msk||_0 > ||\fst||_0$.
% % that three inequalities hold:
% % \begin{enumerate}
% %     \item The number of 1s in $\xpi{f}^T > \ceil*{l/2}$. 
% %     \item The number of 1s in ($\msk - \fst$) $> \ceil*{l/2}$.
% %     \item This relationship holds with respect to the number: (number of coinciding locations of 1s in $\xpi{f}^T$ and -1s in ($\msk - \fst$) $<$ (number of coinciding locations of 1s in $\xpi{f}^T$ and 1s in ($\msk - \fst$).
% % \end{enumerate}

% We reduce \ft, $\msk$, and $\fst$ to binary vectors, that is, vectors composed of 0s and 1s. Let $\Delta f = \msk - \fst$. We denote the number of 1s and -1s in $\Delta f$ as $A$ and $B$, respectively. Further, let $p_a$ and $p_b$ denote the number of $(1,1)$ pairs and $(1,-1)$ pairs in \ft and $\Delta f$, respectively. A $(1,1)$ pair in a pair of vectors is defined as having $1$ in the same coordinate of the two vectors. A $(1,-1)$ pair is similarly defined. From the definitions, we have $0<p_a<A$ and $0<p_b<B$.

% \noindent Goal: $p_b < p_a$ for all $p_b$
% % (condition 3 in Section 4.2.1 for Lemma 1) implies Lemma 1 is true. Now, suppose $A \leq B$. Then $p_b > p_a$ for $0<A<p_b<B$. This gives rise to a contradiction. Therefore, $A>B$. Now let $x$ and $y$ denote the number of 1s in $\msk$ and $\fst$, respectively. Then $x \geq A$ and $y\geq B$. If $y=B$, then $x\geq A > B = y \implies x > y$. If $y>B$, then $A \gets A - (y - B)$. But $A>B \implies A - (y-B)>B \implies A>y$. Since $x\geq A$, $x>y$. Hence, $A>B \implies x>y$.

% % \noindent In the backward direction, 
%  Now let $x$ and $y$ denote the $L_0$ norm of $\msk$ and $\fst$, respectively. From our padding procedure, we have $x>y$. Then, if $y = B$, then $x=A$ and $A>B$. But if $y>B$, then $A= x-(y-B) \implies A - B = x - y$. From $x>y$, it follows that $A>B$. Thus, $x>y \implies A>B$.

% \end{proof}

% \vspace{-10pt}
% \begin{proof}

% In our approach, we use Mask R-CNN for pedestrian detection, which outputs bounding boxes and their corresponding masks. We use the mask and bounding box pair to generate a segmented box (Section 4.1.1). In practice, a segmented box produces ``more descriptive" appearance features with a lower cosine cost than bounding boxes (lemma \ref{lemma1}). The correct assignment of an ID depends on successful feature matching between the predicted measurement feature and the optimal detection feature. Equivalently, 

% \begin{equation}
% \mathnormal{d}(\xpi{f},f_{h^{*}_{j,{\p}}})>\lambda \Leftrightarrow \alpha_{\p} = \phi, \forall \p.
% \label{eqn:assign}
% \end{equation} 
    
    
% \noindent Using Lemma \ref{lemma1} and the fact that $\lambda \underset{i.i.d.}{\sim} \bb{U}[0,1]$, 
% \[\bb{P}(\mathnormal{d}(\xpi{f} , f^M_{h^{*}_{j,\p}} ) > \lambda) < \bb{P}(\mathnormal{d}(\xpi{f} ,f^F_{h^{*}_{j,\p}} ) > \lambda), \forall \p,\] 
% \noindent Using (\ref{eqn:assign}), it directly follows that,
% \begin{equation}
%     \bb{P}^M(\alpha_{\p} = \phi) < \bb{P}^F(\alpha_{\p} = \phi), \forall \p.
%     \label{alpha}
% \end{equation}


% \noindent In our approach, we set \[(\mu>\xi) \land  (\alpha_{\p} = \phi) \Leftrightarrow \mc{T}_{t,\p} \gets \{\phi\}\]
% Using (\ref{alpha}), it follows that,
% \begin{equation}
% \bb{P}^M(\mc{T}_{t,\p} \gets \{\phi\}) < \bb{P}^F(\mc{T}_{t,\p} \gets \{\phi\}), \forall \p
% \label{prob}
% \end{equation}

% \noindent We define the total number of false negatives (FN) as 
% \begin{equation}
%     FN = \sum_{t=1}^T \sum_{p_g \in \mc{G}} \delta_{\mc{T}_{t,p_g}}
%     \label{fn}
% \end{equation}
% where $p_g \in \mc{G}$ denotes a ground truth pedestrian in the set of all ground truth pedestrians in $\bb{F}_t$ and $\delta_z = 1$ for $z=0$ and 0 elsewhere, which is a variation of the Kronecker delta function.
% Using (\ref{prob}) and (\ref{fn}), we can say that fewer lost tracks ($\mc{T}_{t,\p} \gets \{\phi\}$) indicate a smaller number of false negatives. Finally, by using Lemma \ref{lemma1} with the association formulation (\ref{optim}) described in the next subsection, it is easy to see that $\bb{P}^M(\Gamma(\alpha_{\p}))>\bb{P}^F(\Gamma(\alpha_{\p}))$, which completes the proof.
% \end{proof}

% The upper bound, $\bb{P}^F(\mc{T}_{t,\p})$, in \ref{prob} depends on the amount of padding done to $\xpi{f}$ and $\xhj{f}$. A general observed trend is that a higher amount of padding results in a larger bound in Equation (\ref{prob}).

We explain the proof in detail in [mention link.



==> notation.tex <==
% \subsection{Notation}
% Throughout the rest of this paper, we use the following notation. A frame at a given time $t$ is denoted by $\bb{F}_t$ and a sequence of frames until time $t$, by $\bb{F}_{1:t}$. In every $\bb{F}_t$, let $\p$ denote the $\ith$ agent and $\h$ denote the $\jth$ detected agent. Further, $\xpi{f}$ and $\xhj{f}$ denote the feature vector of $\p$ and $\h$, respectively. $T$ denotes the total number of frames in the image sequence and $N_t$ represents the total number of road-agents in $\bb{F}_t$. $\bb{R}(\cdot)$ denotes the range. $\mc{H}$ is the set of all agent detections in $\bb{F}_t$ and $\mc{P}$ is the set of all road-agents in $\bb{F}_t$. $r$ is a predefined radius around every $\p$ and $\mc{H}_i$ is the set of all detected road-agents within a circle of radius $r$ centered around $\p$. $N_i$ is the number of such detected road-agents. Thus, $\mc{H} = \{ \h \ | \ j \in \bb{R}(N_t) \}, \mc{H}_i = \{ \h \ | \ r \geq |\p - \h|, i \in \bb{R}(N_i) \},$ and $\mc{P} = \{ \p \ | \ i \in \bb{R}(N_t) \}$, where $i$ and $j$ denote the indices of road-agents and detections, respectively. Finally, the Cosine metric \cite{cosine} measures the dot product between two vector quantities, $a$ and $b$. It is mathematically defined as $\mathnormal{l}(a,b) = 1 - a^Tb$.


\begin{table}
  \centering
  \resizebox{\columnwidth}{!}{
  \scalebox{0.4}{
  \begin{tabular}{|c|l|}
  \hline
    Symbol  & Description \\
    \hline
    $\p$& $i^{\tim{th}}$ agent.\\
    $\h$& $j^{\tim{th}}$ detected agent (ie, it has a bounding box).\\
    % $\bb{F}_t$& current frame at timestep $t$\\
    $\mc{P}$& set of all road-agents in the current frame.\\
    $\mc{H}$& set of all detected road-agents in the current frame.\\
    $\mc{H}_i$& subset of all unmatched detected road-agents in the current frame \\
             & that are within a circular region around agent $\p$.\\
    $\bb{B_{\p}}, \bb{B_{\h}}$& bounding box for the predicted state of a pedestrian $\p$, and a detected agent $\h$, respectively.\\
    $p_i \equiv (u_i,v_i)$ & position of $\p$, similarly defined for $p_k$.\\
    $\nu_i \equiv (\Dot{u}_i, \Dot{v}_i)$ & velocity of $\p$, similarly defined for $p_k$.\\
    $f_{\p}$ & feature vectors of the predicted agent, $\p$. \\
    $ f_{\h}$ & feature vectors of the segmented representation, $\h$.\\
    $l(x,y)$& cosine metric defined by $1 - x^Ty$.\\
    $\Psi_{t}$ & state of an agent $\p$ at time $t$, includes position, \\& velocity, and preferred velocity.\\
    $w$ & width of bounding box for detected agent $\h$.\\
    $h$ & height of bounding box for detected agent $\h$.\\
    \hline
  \end{tabular}
  }
  }
  \caption{Notations used in the paper. }
  \vspace{-15pt}
  \label{table0}
\end{table}


